Modeling Multi-Vehicle Interaction Scenarios Using Gaussian Random Field

Autonomous vehicles are expected to navigate in complex traffic scenarios with multiple surrounding vehicles. The correlations between road users vary over time, the degree of which, in theory, could be infinitely large, thus posing a great challenge in modeling and predicting the driving environment. In this paper, we propose a method to model multi-vehicle interactions using a stochastic vector field model and apply non-parametric Bayesian learning to extract the underlying motion patterns from a large quantity of naturalistic traffic data. We then use this model to reproduce the high-dimensional driving scenarios in a finitely tractable form. We use a Gaussian process to model multi-vehicle motion, and a Dirichlet process to assign each observation to a specific scenario. We verify the effectiveness of the proposed method on highway and intersection datasets from the NGSIM project, in which complex multi-vehicle interactions are prevalent. The results show that the proposed method can capture motion patterns from both settings, without imposing heroic prior, and hence demonstrate the potential application for a wide array of traffic situations. The proposed modeling method could enable simulation platforms and other testing methods designed for autonomous vehicle evaluation, to easily model and generate traffic scenarios emulating large scale driving data.

==> Notation.tex <==
\section{Notation}
\begin{table}[!h]
\caption{ \label{notation}}
\centering
\begin{tabular}{|p{0.08\textwidth}|p{0.3\textwidth}|}
\hline
s & Each observation/frame of data consisting of 4 arrays: $V^{s}_{x}, V^{s}_{y}, X^{s}, Y^{s}$\\
\hline
g & Motion pattern \\
\hline
$z_{i}$ & Index of motion pattern assigned to frame $s_{i}$\\
\hline
$n_{k}$ & Count of frames assigned to motion pattern $g_{k}$\\
\hline
N & Total number of frames\\
\hline
K & Number of motion patterns\\
\hline
k & Index of motion pattern\\
\hline
$\alpha$ & concentration parameter\\
\hline
a & Shape parameter for gamma prior of w; constant \\
 \hline
b & Scale parameter for gamma prior of w; constant \\
 \hline
\end{tabular}
\end{table}
